A Unified Continual Learning Framework with General Parameter-Efficient Tuning

The "pre-training $\rightarrow$ downstream adaptation" presents both new opportunities and challenges for Continual Learning (CL). Although the recent state-of-the-art in CL is achieved through Parameter-Efficient-Tuning (PET) adaptation paradigm, only prompt has been explored, limiting its application to Transformers only. In this paper, we position prompting as one instantiation of PET, and propose a unified CL framework with general PET, dubbed as Learning-Accumulation-Ensemble (LAE). PET, e.g., using Adapter, LoRA, or Prefix, can adapt a pre-trained model to downstream tasks with fewer parameters and resources. Given a PET method, our LAE framework incorporates it for CL with three novel designs. 1) Learning: the pre-trained model adapts to the new task by tuning an online PET module, along with our adaptation speed calibration to align different PET modules, 2) Accumulation: the task-specific knowledge learned by the online PET module is accumulated into an offline PET module through momentum update, 3) Ensemble: During inference, we respectively construct two experts with online/offline PET modules (which are favored by the novel/historical tasks) for prediction ensemble. We show that LAE is compatible with a battery of PET methods and gains strong CL capability. For example, LAE with Adaptor PET surpasses the prior state-of-the-art by 1.3% and 3.6% in last-incremental accuracy on CIFAR100 and ImageNet-R datasets, respectively. Code is available at \url{https://github.com/gqk/LAE}.

==> figure/benchmark_imagenet-r_t20.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{file/imagenet-r-init10-inc10.pdf}
  \end{center}
  \vskip -0.1in
  \caption{Task-by-Task Incremental Accuracy on 20-Task ImageNet-R Benchmark. The lines show the task-by-task evaluation results of L2P~\cite{l2p}, DualPrompt~\cite{dual_prompt}, ENS~\cite{esn}, and our LAE framework with different PET modules.}
  \label{fig:benchmark_imr}
\end{figure}
